Deformation Patterns and Surface Morphology in a Minimal Model of Amorphous Plasticity

We investigate a minimal model of the plastic deformation of amorphous materials. The material elements are assumed to exhibit ideally plastic behavior (J2 plasticity). Structural disorder is considered in terms of random variations of the local yield stresses. Using a finite element implementation of this simple model, we simulate the plane-strain deformation of long thin rods loaded in tension. The resulting strain patterns are statistically characterized in terms of their spatial correlation functions. Studies of the corresponding surface morphology reveal a non-trivial Hurst exponent of approx. 0.8, indicating the presence of long range correlations in the deformation patterns. The simulated deformation patterns and surface morphology exhibit persistent features which emerge already at the very onset of plastic deformation, while subsequent evolution is characterized by growth in amplitude without major morphology changes. The findings are compared to experimental observations.

==> makefile <==

# -----------------------------------------------------------------------------
# Paths and Filenames
# -----------------------------------------------------------------------------
texfile=surface_morphology.tex
somfile=

bname=$(basename $(texfile))
PF="`date +%y-%m-%d`_"
zipname=$(PF)$(basename $(texfile))

# only used for zip
#bibfile=paper.bib

# -----------------------------------------------------------------------------
# Rules and Commands
# -----------------------------------------------------------------------------
LATEX=pdflatex -src-specials
BIBTEX=bibtex
RM=rm -f

%.bbl: %.aux
	$(BIBTEX) $<




# -----------------------------------------------------------------------------
# Targets
# -----------------------------------------------------------------------------
default:
	@$(MAKE) paper
#	@$(MAKE) paper som

help:
	@echo
	@echo "=================================================================="
	@echo " usage: make [option]"
	@echo " You can use the following options with this makefile:"
	@echo "=================================================================="
	@echo "  [default]     (= no option given)"
	@echo "                makes the paper and som"
	@echo
	@echo "  paper         makes the paper"
	@echo 
	@echo "  clean         removes all temp. and pdf files in this directory"
	@echo 
	@echo "  cleanaux      as 'clean' but removes additinally all eps figures"
	@echo "                and temporary files"
	@echo 
	@echo "  zip           creates a zipped directory with all required files"
	@echo 
	@echo "  all           make figures, the paper and som"
	@echo "                !! making figures can take a while and requires !!"
	@echo "                !! the matplotlib and SUtils libraries          !!"
	@echo "=================================================================="


all: 
	@$(MAKE) figures paper



paper:
	$(MAKE) pdf





# produce bending pictures



bibliography: 
	$(BIBTEX) $(bname)



pdf: 	
	$(LATEX) $(texfile) 2>/dev/null || { $(RM) $(bname).dvi $(bname).aux && false ; }
	while grep 'Rerun to get' $(bname).log ; do \
	   $(LATEX) $(texfile) 2>/dev/null || { $(RM) $(bname).pdf $(bname).aux && false ; } ; \
	done



.PHONY: figures
figures:
	cd figures; make 


figureclean:
	cd figures; make clean




clean:
	-$(RM) $(bname).dvi $(bname).pdf $(bname).spl *.aux *.log *.toc *.bbl *.blg *.pfg *~  *Notes.bib 


cleanaux:
	@make clean figureclean
	-$(RM) $(bname).tex.backup

tgz:
#	make figures
	make paper
	mkdir -p $(zipname)/figures
	cp  figures/*.png  figures/system.pdf   $(zipname)/figures/.
	cp $(texfile)                           $(zipname)/$(texfile)
	cp makefile  iopams.sty  *.clo *.cls    $(zipname)
	chmod 777 $(zipname)/makefile
#	cd $(zipname) && zip -r $(zipname).zip * && mv $(zipname).zip ..
	tar czvf $(zipname).tgz $(zipname)


# zip file without root-subdirectory for submission!!
# the figures must have been made before!
jstat_zip:
	mkdir -p $(zipname)/figures
	cp  figures/*.png  figures/system.pdf   $(zipname)/figures/.
	cp $(texfile)                           $(zipname)/$(texfile)
	cp  iopams.sty  *.clo *.cls    $(zipname)
	cd $(zipname) && zip -r $(zipname).zip * && mv $(zipname).zip ..
#	tar czvf $(zipname).tgz $(zipname)

